Modeling turbulent wave-front phase as a fractional Brownian motion: a new approach

This paper introduces a general and new formalism to model the turbulent wave-front phase using fractional Brownian motion processes. Moreover, it extends results to non-Kolmogorov turbulence. In particular, generalized expressions for the Strehl ratio and the angle-of-arrival variance are obtained. These are dependent on the dynamic state of the turbulence.

==> pstricks-add.tex <==
%%
%% This is file `pstricks-add.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pstricks-add.tex'
%%
%% Herbert Voss <voss@perce.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pstricks-add' is a PSTricks package for additionals to the standard
%%         pstricks package
%%
\def\fileversion{0.9a}
\let\pstricksAddFV\fileversion
\def\filedate{2003/10/15}
\message{`pstricks-add' v\fileversion, \filedate\space (Herbert Voss)}
\csname PSTricksAddLoaded\endcsname
\let\PSTricksAddLoaded\endinput
% Requires PSTricks, pst-node
\usepackage{pstcol}
\ifx\PSTricksLoaded\endinput\else\input pstricks \fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node \fi
\usepackage{multido}
%
\input pst-key
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor
%
% a new fillstyle
\def\psfs@asolid{\pst@fill{\pst@usecolor\psfillcolor eofill}}
%
\define@key{psset}{braceWidth}{\edef\psk@braceWidth{#1}}
\define@key{psset}{bracePos}{\edef\psk@bracePos{#1}}
\setkeys{psset}{braceWidth=0.35,bracePos=0.5}
%
\def\@@rput@iv(#1){\pst@killglue\pst@makebox{\@@rput@v{#1}}}
\def\@@rput@v#1{%
	\begingroup
		\use@par
		\pst@makesmall\pst@hbox
		\pst@Verb{%
			Alpha 90 sub \psk@braceWidth\space 0 lt {180 add} if
			\ifx\psk@rot\@empty\else\psk@rot add \fi
			/rotAngle exch def
		}%
		\setbox\pst@hbox=\hbox{%
			\pst@Verb{rotAngle \tx@RotBegin}%
			\box\pst@hbox\pst@Verb{\tx@RotEnd}%
		}%
		\psput@{#1}\pst@hbox
	\endgroup
	\ignorespaces%
}
%
\def\psbrace{\@ifnextchar[{\@psbrace}{\@psbrace[]}}
\def\@psbrace[#1](#2)(#3)#4{{
	\setkeys{psset}{linearc=0.2,linewidth=1pt,%
		nodesepA=0pt,nodesepB=0pt,bracePos=0.5}% the default
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa%
	\pst@getcoor{#3}\pst@tempb%
	\pnode(!%
		/bW2 \psk@braceWidth\space 2.0 div def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/Alpha YB YA sub XB XA sub atan def
		/xMid XB XA sub \psk@bracePos\space mul XA add def
		/yMid YB YA sub \psk@bracePos\space mul YA add def
		/@deltaX Alpha sin bW2 mul def
		/@deltaY Alpha cos bW2 mul def
		/@xTemp xMid @deltaX 2 mul add def
		/@yTemp yMid @deltaY 2 mul sub def
		@xTemp @yTemp){@tempNode}
	\pst@getcoor{@tempNode}\pst@tempc%
	\@@rput@iv(! %
		\pst@tempc /Yc exch def
		/Xc exch def
		Xc \psk@nodesepA\space add \pst@number\psxunit div
		Yc \psk@nodesepB\space add \pst@number\psxunit div ){#4}
	\psline(#2)%
		(! XA @deltaX add YA @deltaY sub)%
		(! @xTemp @deltaX sub @yTemp @deltaY add)%
		(@tempNode)
	\psline(@tempNode)%
		(! @xTemp @deltaX sub @yTemp @deltaY add)%
		(! XB @deltaX add YB @deltaY sub)%
		(#3)%
}}
%
% from Dennis Giroux: http://www.tug.org/pipermail/pstricks/2001/000507.html
%
% I - Definition of \PstWedgeEllipse, a generalization of \pswedge for wedges
%     of ellipses (from the code of \pswedge and \psellipse)
%
\def\psWedgeEllipse{\def\pst@par{}\pst@object{psWedgeEllipse}}
\def\psWedgeEllipse@i(#1){%
	\@ifnextchar({\psWedgeEllipse@ii(#1)}{\pstWedgeEllipse@ii(0,0)(#1)}}
\def\psWedgeEllipse@ii(#1)(#2)#3#4{%
	\begin@ClosedObj
		\pst@getangle{#3}\pst@tempa
		\pst@getangle{#4}\pst@tempb
		\pst@getcoor{#1}\pst@tempc
		\pst@@getcoor{#2}%
		\def\pst@linetype{1}%
		\addto@pscode{%
			\pst@tempa \pst@tempb
			\pst@coor
			\pst@tempc moveto
			\ifdim\psk@dimen\p@=\z@\else
				\psk@dimen CLW mul dup 3 1 roll
				sub 3 1 roll sub exch
			\fi
			\pst@tempc
			\tx@Ellipse
			closepath%
		}%
		\showpointsfalse
	\end@ClosedObj%
}
%
% arcs
%
\def\psEllipticArcN{\def\pst@par{}\pst@object{psellipticarcn}}
\def\psellipticarcn@i{\let\if@psarcn\iftrue\psellipticarc@ii}
%
\def\psEllipticArc{\def\pst@par{}\pst@object{psellipticarc}}
\def\psellipticarc@i{\let\if@psarcn\iffalse\psellipticarc@ii}
%
\let\if@psarcn\iffalse
\def\psellipticarc@ii{\pst@getarrows\psellipticarc@iii}
\def\psellipticarc@iii(#1){%
	\@ifnextchar({\psellipticarc@iv(#1)}{\psellipticarc@iv(0,0)(#1)}}
\def\psellipticarc@iv(#1)(#2)#3#4{%
	\begin@OpenObj
		\pst@getcoor{#1}\pst@tempa
		\pst@getcoor{#2}\pst@tempb
		\pst@getangle{#3}\pst@tempc
		\pst@getangle{#4}\pst@tempd
		\addto@pscode{\psellipticarc@definearg \psellipticarc@draw}%
		\showpointsfalse
	\end@OpenObj%
}
\def\psellipticarc@definearg{%
	\pst@tempa /y ED /x ED  % Origin
	\pst@tempb              % radii. Now adjust:
	\ifdim\psk@dimen\p@=\z@\else
		\psk@dimen CLW mul dup 3 1 roll
		sub 3 1 roll sub exch
	\fi
	/ry ED /rx ED
	/angleA
		/d  {  \if@psarcn sub \else add \fi } def
		\pst@tempc \psk@arcsepA 2 div
		\tx@ArcAdjust
	def
	/angleB
		/d  {  \if@psarcn add \else sub \fi } def
		\pst@tempd \psk@arcsepB 2 div
		\tx@ArcAdjust
	def
	\ifshowpoints\psellipticarc@showpoints\fi
	\ifx\psk@arrowA\@empty
		\ifnum\psk@liftpen=2
			angleA cos rx mul x add
			angleA sin ry mul y add
			moveto
		\fi
	\fi%
}
\def\psellipticarc@draw{%
	0 0 1
	angleA
	\ifx\psk@arrowA\@empty\else
		{ ArrowA CP }
		{ \if@psarcn sub \else add \fi }
		\tx@EllipticArcArrow
	\fi
	angleB
	\ifx\psk@arrowB\@empty\else
		{ ArrowB }
		{ \if@psarcn add \else sub \fi }
		\tx@EllipticArcArrow
	\fi
	/mtrx CM def
	x y T
	rx ry scale
	\if@psarcn arcn \else arc \fi
	mtrx setmatrix%
}
\def\psellipticarc@showpoints{%
	gsave
	/mtrx CM def
	x y T
	rx ry scale
	0 0 moveto
	0 0 1 \pst@tempc \pst@tempd
	\ifcase\psarc@type arc \or arcn \fi
	closepath
	mtrx setmatrix
	CLW 2 div SLW
	[ \psk@dash\space ] 0 setdash stroke
	grestore %
}
\pst@def{ArcAdjust}<%
% given a target length (targetLength) and an initial angle (angle0) [in the stack],
% let  M(angle0)=(rx*cos(angle0),ry*sin(angle0))=(x0,y0).
% This computes an angle t such that (x0,y0) is at distance targetLength from the point M(t)=(rx*cos(t),ry*sin(t)).
% NOTE: this an absolute angle, it does not have to be added or substracted to angle0
% contrary to TvZ's code.
% To achieve, this, one iterates the following process: start with some angle t,
% compute the point M' at distance targetLength of (x0,y0) on the semi-line [(x0,y0) M(t)].
% Now take t' (= new angle) so that (0,0) M(t') and M' are aligned.
%
% Another difference with TvZ's code is that we need d (=add/sub) to be defined.
% the value of d = add/sub is used to know on which side we have to move.
% It is only used in the initialisation of the angle before the iteration.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Input stack:  1: target length 2: initial angle
% variables used : rx, ry, d (=add/sub)
%
	/targetLength ED /angle0 ED
	/x0 rx angle0 cos mul def
	/y0 ry angle0 sin mul def
% we are looking for an angle t such that (x0,y0) is at distance targetLength from the point M(t)=(rx*cos(t),ry*sin(t)))
%initialisation of angle (using 1st order approx = TvZ's code)
	targetLength 57.2958 mul
	angle0 sin rx mul dup mul
	angle0 cos ry mul dup mul
	add sqrt div
% if initialisation angle is two large (more than 90 degrees) set it to 90 degrees
% (if the ellipse is very curved at the point where we draw the arrow, the value can be much more than 360 degrees !)
% this should avoid going on the wrong side (more than 180 degrees) or go near
% a bad attractive point (at 180 degrees)
	dup 90 ge { pop 90 } if
	angle0 exch d
% maximum number of times to iterate the iterative procedure:
	30
% iterative procedure: takes an angle t on top of stack, computes a better angle (an put it on top of stack)
	{ dup
% compute distance D between (x0,y0) and M(t)
	dup cos rx mul x0 sub dup mul exch sin ry mul y0 sub dup mul add sqrt
% if D almost equals targetLength, we stop
	dup targetLength sub abs 1e-5 le { pop exit } if
% stack now contains D t
% compute the point M(t') at distance targetLength of (x0,y0) on the semi-line [(x0,y0) M(t)]:
% M(t')= ( (x(t)-x0)*targetLength/d+x0 , (y(t)-y0)*targetLength/d+y0 )
	exch dup cos rx mul x0 sub  exch sin ry mul y0 sub
% stack contains:  y(t)-y0, x(t)-x0, d
	2 index \tx@Div targetLength mul y0 add ry \tx@Div exch
	2 index \tx@Div targetLength mul x0 add rx \tx@Div
% stack contains x(t')/rx , y(t')/ry , d
% now compute t', and remove D from stack
	atan exch pop
	} repeat
% we don't look at what happened... in particular, if targetLength is greater than the diameter of the ellipse...
% the final angle will be around /angle0 + 180. maybe we should treat this pathological case...
%after iteration, stack contains an angle t such that M(t) is the tail of the arrow
% to give back the result as a an angle relative to angle0 we could add the following line:
% angle0 sub 0 exch d
>
\pst@def{EllipticArcArrow}<%
	/d ED      % add/sub
	/b ED      % arrow procedure
	/a1 ED     % angle
	gsave
	newpath
	0 -1000 moveto
	clip                  % Set clippath far from arrow.
	newpath
	0 1 0 0 b             % Draw arrow to determine length.
	grestore
% Length of arrow is on top of stack. Next 3 numbers are junk.
%
	a1 exch \tx@ArcAdjust   % Angular position of base of arrow.
	/a2 ED
	pop pop pop
	a2 cos rx mul x add
	a2 sin ry mul y add
	a1 cos rx mul x add
	a1 sin ry mul y add
	% Now arrow tip coor and base coor are on stack.
	b pop pop pop pop       % Draw arrow, and discard coordinates.
	a2 CLW 8 div
% change value of d (test it by looking if  `` 1 1 d '' gives 2 or not )
	1 1 d 2 eq { /d { sub } def } { /d { add } def } ifelse
	\tx@ArcAdjust
% resets original value of d
	1 1 d 2 eq { /d { sub } def } { /d { add } def } ifelse>  % Adjust angle to give overlap.
%

%
% -------------- the arrow part -------------
%  the original table
% \def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-]}
\edef\pst@arrowtable{\pst@arrowtable,)-(,]-[,|>-<|}
%
\@namedef{psas@<|}{%
    \psk@tbarsize \tx@Tbar
    0 CLW 2 div T
    newpath
    true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow%
}
% ]-[ arrow
\def\tx@BracketOut{BracketOut }
\@namedef{psas@[}{%
	/BracketOut {%
	CLW mul add dup CLW sub 2 div
%/x ED mul CLW add
	/x ED mul neg
	/y ED
	/z CLW 2 div def
	x neg y moveto
	x neg CLW 2 div L x CLW 2 div L x y L stroke 0 CLW moveto } def
	\psk@bracketlength \psk@tbarsize \tx@BracketOut
}
% )-( arrow
\def\tx@RoundBracketOut{RoundBracketOut }
\@namedef{psas@(}{%
	/RoundBracketOut {%
	CLW mul add dup 2 div
%/x ED mul
	/x ED mul neg
	/y ED
	/mtrx CM def
	0 CLW
	2 div T x y mul 0 ne { x y scale } if
	1 1 moveto
	.85 .5 .35 0 0 0 curveto
	-.35 0 -.85 .5 -1 1 curveto
	mtrx setmatrix stroke 0 CLW moveto } def
	\psk@rbracketlength \psk@tbarsize \tx@RoundBracketOut
}
%
% Redefininition of \psset@arrowscale to store value of X scale factor
\def\psset@arrowscale#1{\pst@getscale{#1}\psk@arrowscale}
\psset@arrowscale{1}

\def\psset@arrowscale#1{%
	\psset@arrowscale@i#1 \@nil
	\pst@getscale{#1}\psk@arrowscale%
}
\def\psset@arrowscale@i#1 #2\@nil{\edef\pst@arrowscale{#1}}
\def\pst@arrowscale{1}

% New parameter "arrowfill", with default as "true"
\newif\ifpsArrowFill
\def\psset@ArrowFill#1{\@nameuse{psArrowFill#1}}
\psset@ArrowFill{true}

% Modification of the PostScript macro Arrow to choose to fill or not the arrow
% (it require to restore the current linewidth, despite of the scaling)
\pst@def{Arrow}<{%
    CLW mul add dup 2 div
    /w ED mul dup
    /h ED mul
    /a ED { 0 h T 1 -1 scale } if
    gsave
    \ifpsArrowFill\else
	\pst@number\pslinewidth \pst@arrowscale\space div SLW
    \fi
    w neg h moveto
    0 0 L w h L w neg a neg rlineto
    \ifpsArrowFill gsave fill grestore \else gsave closepath stroke grestore \fi
	grestore
	0 h a sub moveto
}>
\@namedef{psas@>>}{%
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h a sub T
    gsave
    newpath
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    CP
    grestore
    moveto
}
%
\@namedef{psas@<<}{%
    true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h neg a add T
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h a 5 mul 2 div sub moveto
}
%
% DG addition begin - Dec. 18/19, 1997 and Oct. 11, 2002
% Adapted from \psset@arrows
\def\psset@ArrowInside#1{%
    \begingroup
		\pst@activearrows
		\xdef\pst@tempg{<#1}%
    \endgroup
    \expandafter\psset@@ArrowInside\pst@tempg\@empty-\@empty\@nil
    \if@pst\else
		\@pstrickserr{Bad intermediate arrow specification: #1}\@ehpa
    \fi%
}
% Adapted from \psset@@arrows
\def\psset@@ArrowInside#1-#2\@empty#3\@nil{%
    \@psttrue
    \def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
    \expandafter\next\pst@arrowtable,#1-#1,\@nil
    \@ifundefined{psas@#2}%
		{\@pstfalse\def\psk@ArrowInside{}}%
		{\def\psk@ArrowInside{#2}}%
}
% Default value empty
\def\psk@ArrowInside{}
% Modified version of \pst@addarrowdef
\def\pst@addarrowdef{%
    \addto@pscode{%
		/ArrowA {
			\ifx\psk@arrowA\@empty
				\pst@oplineto
			\else
				\pst@arrowdef{A}
				moveto
			\fi
		} def
		/ArrowB {
			\ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi
		} def
% DG addition
		/ArrowInside {
			\ifx\psk@ArrowInside\@empty \else \pst@arrowdefA{Inside} \fi
		} def
	}%
}
% Adapted from \pst@arrowdef
\def\pst@arrowdefA#1{%
	\ifnum\pst@repeatarrowsflag>\z@
		/Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
	\fi
	\tx@BeginArrow
	\psk@arrowscale
	\@nameuse{psas@\@nameuse{psk@Arrow#1}}
	\tx@EndArrow%
}
% ArrowInsidePos parameter (default value 0.5)
\def\psset@ArrowInsidePos#1{\pst@checknum{#1}\psk@ArrowInsidePos}%
\psset@ArrowInsidePos{0.5}
%
% Modified version of \begin@ClosedObj
\def\begin@ClosedObj{%
    \leavevmode
    \pst@killglue
    \begingroup
	\use@par
	\solid@star
	\ifpsdoubleline \pst@setdoublesep \fi
	\pst@addarrowdef% DG addition
	\init@pscode
}
%
% Redefinition of the PostScript /Line macro to print the intermediate
% arrow on each segment of the line
%
\def\psset@ArrowInsideNo#1{\pst@checknum{#1}\psk@ArrowInsideNo}% hv 20031001
\def\psset@ArrowInsideOffset#1{\pst@checknum{#1}\psk@ArrowInsideOffset}% hv 20031001
\psset{ArrowInsideNo=1,ArrowInsideOffset=0}
%
\pst@def{Line}<{%
	NArray n 0 eq not { n 1 eq { 0 0 /n 2 def } if
    (\psk@ArrowInside) length 0 gt {
		2 copy /y1 ED /x1 ED ArrowA x1 y1
    	/n n 1 sub def
    	n {
			4 copy
			/y1 ED /x1 ED /y2 ED /x2 ED
			x1 y1
			\psk@ArrowInsidePos\space 1 gt{
				/Alpha y2 y1 sub x2 x1 sub atan def
				/ArrowPos \psk@ArrowInsideOffset\space def
				/Length x2 x1 sub y2 y1 sub Pyth def
				/dArrowPos \psk@ArrowInsidePos\space abs def
				{
					/ArrowPos ArrowPos dArrowPos add def
					ArrowPos Length gt { exit } if
					x1 Alpha cos ArrowPos mul add
					y1 Alpha sin ArrowPos mul add
					ArrowInside
					pop pop
				} loop
			}{
				/ArrowPos \psk@ArrowInsideOffset\space def
				/dArrowPos \psk@ArrowInsideNo 1 gt {%
					1.0 \psk@ArrowInsideNo 1.0 add div
				}{ \psk@ArrowInsidePos } ifelse def
				\psk@ArrowInsideNo\space cvi {
					/ArrowPos ArrowPos dArrowPos add def
					x2 x1 sub ArrowPos mul x1 add
					y2 y1 sub ArrowPos mul y1 add
					ArrowInside
					pop pop
				} repeat
			} ifelse
			pop pop Lineto
		} repeat
	}{ ArrowA /n n 2 sub def n { Lineto } repeat } ifelse
	CP 4 2 roll ArrowB L pop pop } if%
}>
%
% Redefinition of the PostScript /Polygon macro to print the intermediate
% arrow on each segment of the line
\pst@def{Polygon}<{%
	NArray n 2 eq { 0 0 /n 3 def } if
	n 3 lt {
		n { pop pop } repeat
	}{
		n 3 gt { CheckClosed } if
		n 2 mul
		-2 roll
		/y0 ED
    	/x0 ED
    	/y1 ED
    	/x1 ED
    	/xx1 x1 def
    	/yy1 y1 def
    	x1 y1
    	/x1 x0 x1 add 2 div def
    	/y1 y0 y1 add 2 div def
    	x1 y1 moveto
    	/n n 2 sub def
		/drawArrows {
			x11 y11
			\psk@ArrowInsidePos\space 1 gt {
				/Alpha y12 y11 sub x12 x11 sub atan def
				/ArrowPos \psk@ArrowInsideOffset\space def
				/Length x12 x11 sub y12 y11 sub Pyth def
				/dArrowPos \psk@ArrowInsidePos\space abs def
				{
					/ArrowPos ArrowPos dArrowPos add def
					ArrowPos Length gt { exit } if
					x11 Alpha cos ArrowPos mul add
					y11 Alpha sin ArrowPos mul add
					ArrowInside
					pop pop
				} loop
			}{
				/ArrowPos \psk@ArrowInsideOffset\space def
				/dArrowPos \psk@ArrowInsideNo 1 gt {%
					1.0 \psk@ArrowInsideNo 1.0 add div
				}{ \psk@ArrowInsidePos } ifelse def
					\psk@ArrowInsideNo cvi {
					/ArrowPos ArrowPos dArrowPos add def
					x12 x11 sub ArrowPos mul x11 add
					y12 y11 sub ArrowPos mul y11 add
        			ArrowInside
					pop pop
				} repeat
			} ifelse
			pop pop Lineto
		} def
		n {
			4 copy
			/y11 ED /x11 ED /y12 ED /x12 ED
			drawArrows
		} repeat
		x1 y1 x0 y0
		6 4 roll
		2 copy
		/y11 ED /x11 ED /y12 y0 def /x12 x0 def
		drawArrows
		/y11 y0 def /x11 x0 def /y12 yy1 def /x12 xx1 def
		drawArrows
		pop pop
    	closepath
	} ifelse %
}>
%
%
% Redefinition of the PostScript /OpenBezier macro to print the intermediate
% arrow
\pst@def{OpenBezier}<{%
	/dArrowPos \psk@ArrowInsideNo 1 gt {%
		1.0 \psk@ArrowInsideNo 1.0 add div
	}{ \psk@ArrowInsidePos } ifelse def
	BezierNArray
	n 1 eq { pop pop
	}{ 2 copy
		/y0 ED /x0 ED
		ArrowA
		n 4 sub 3 idiv { 6 2 roll 4 2 roll curveto } repeat
		6 2 roll
		4 2 roll
		ArrowB
		/y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
    	/cx x1 x0 sub 3 mul def
		/cy y1 y0 sub 3 mul def
		/bx x2 x1 sub 3 mul cx sub def
		/by y2 y1 sub 3 mul cy sub def
		/ax x3 x0 sub cx sub bx sub def
		/ay y3 y0 sub cy sub by sub def
		/getValues {
			ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
			ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
			ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
			ay t 3 exp mul by t t mul mul add cy t mul add y0 add
		} def
		/getdL {
			getValues
			3 -1 roll sub 3 1 roll sub Pyth
		} def
		/CurveLength {
			/u 0 def
			/du 0.01 def
			0 100 {
				/t0 u def
				/u u du add def
				/t u def
				getdL add
			} repeat } def
		/GetArrowPos {
			/ende \psk@ArrowInsidePos\space 1 gt
				{ArrowPos}
				{ArrowPos CurveLength mul} ifelse def
			/u 0 def
			/du 0.01 def
			/sum 0 def
			{
				/t0 u def
				/u u du add def
		    	/t u def
				/sum getdL sum add def
				sum ende gt {exit} if
			} loop u
		} def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/loopNo \psk@ArrowInsidePos\space 1 gt {%
			CurveLength \psk@ArrowInsidePos\space div cvi
			}{ \psk@ArrowInsideNo } ifelse def
		loopNo cvi {
			/ArrowPos ArrowPos dArrowPos add def
			/t GetArrowPos def
			/t0 t 0.95 mul def
			getValues
			ArrowInside pop pop pop pop
		} repeat
		x1 y1 x2 y2 x3 y3 curveto
	} ifelse
}>
%
% Redefinition of the PostScript /NCLine macro to print the intermediate
% arrow of the line
\pst@def{NCLine}<{%
	NCCoor
	tx@Dict begin
	ArrowA CP 4 2 roll ArrowB
	4 copy
	/y2 ED /x2 ED /y1 ED /x1 ED
	x1 y1
	\psk@ArrowInsidePos\space 1 gt{
		/Alpha y2 y1 sub x2 x1 sub atan def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/Length x2 x1 sub y2 y1 sub Pyth def
		/dArrowPos \psk@ArrowInsidePos\space abs def
		{
			/ArrowPos ArrowPos dArrowPos add def
			ArrowPos Length gt { exit } if
			x1 Alpha cos ArrowPos mul add
			y1 Alpha sin ArrowPos mul add
			ArrowInside
			pop pop
		} loop
	}{
		/ArrowPos \psk@ArrowInsideOffset\space def
		/dArrowPos \psk@ArrowInsideNo 1 gt {%
			1.0 \psk@ArrowInsideNo 1.0 add div
		}{ \psk@ArrowInsidePos } ifelse def
		\psk@ArrowInsideNo\space cvi {
			/ArrowPos ArrowPos dArrowPos add def
			x2 x1 sub ArrowPos mul x1 add
			y2 y1 sub ArrowPos mul y1 add
			ArrowInside
			pop pop
		} repeat
	} ifelse
	pop pop lineto pop pop
	end%
}>
%
\pst@def{NCCurve}<{%
	GetEdgeA GetEdgeB
	xA1 xB1 sub yA1 yB1 sub
	Pyth 2 div dup 3 -1 roll mul
	/ArmA ED
	mul
	/ArmB ED
	/ArmTypeA 0 def
	/ArmTypeB 0 def
	GetArmA GetArmB
	xA2 yA2 xA1 yA1
	2 copy
	/y0 ED /x0 ED
	tx@Dict begin
		ArrowA
	end
	xB2 yB2 xB1 yB1
	tx@Dict begin
		ArrowB
	end
	/y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
	/cx x1 x0 sub 3 mul def
	/cy y1 y0 sub 3 mul def
	/bx x2 x1 sub 3 mul cx sub def
	/by y2 y1 sub 3 mul cy sub def
	/ax x3 x0 sub cx sub bx sub def
	/ay y3 y0 sub cy sub by sub def
	/getValues {
		ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
		ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
		ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
	ay t 3 exp mul by t t mul mul add cy t mul add y0 add
	} def
	/getdL {
		getValues
		3 -1 roll sub 3 1 roll sub Pyth
	} def
	/CurveLength {
		/u 0 def
		/du 0.01 def
		0 100 {
			/t0 u def
			/u u du add def
			/t u def
			getdL add
		} repeat } def
	/GetArrowPos {
		/ende \psk@ArrowInsidePos\space 1 gt {ArrowPos}{ArrowPos CurveLength mul} ifelse def
		/u 0 def
		/du 0.01 def
		/sum 0 def
		{
			/t0 u def
			/u u du add def
			/t u def
			/sum getdL sum add def
			sum ende gt {exit} if
		} loop u
	} def
	/dArrowPos \psk@ArrowInsideNo 1 gt {%
		1.0 \psk@ArrowInsideNo 1.0 add div
	}{ \psk@ArrowInsidePos } ifelse def
	/ArrowPos \psk@ArrowInsideOffset\space def
	/loopNo \psk@ArrowInsidePos\space 1 gt {%
		CurveLength \psk@ArrowInsidePos\space div cvi
		}{ \psk@ArrowInsideNo } ifelse def
	loopNo cvi {
		/ArrowPos ArrowPos dArrowPos add def
		/t GetArrowPos def
		/t0 t 0.95 mul def
		getValues
		ArrowInside pop pop pop pop
	} repeat
	x1 y1 x2 y2 x3 y3 curveto
	/LPutVar [ xA1 yA1 xA2 yA2 xB2 yB2 xB1 yB1 ] cvx def
	/LPutPos { t LPutVar BezierMidpoint } def
	/HPutPos { { HPutLines } HPutCurve } def
	/VPutPos { { VPutLines } HPutCurve } def
}>
%
\def\psset@dashColorI#1{\pst@getcolor{#1}\psDashColorI}
\def\psset@dashColorII#1{\pst@getcolor{#1}\psDashColorII}
\define@key{psset}{dashNo}{\edef\psk@dashNo{#1}}
%
\define@key{psset}{linecap}{\edef\psk@linecap{#1}}
\psset{dashColorI=black,dashColorII=red,dashNo=0.2,linecap=0}
%
\pst@def{LineII}<{%
	NArray
	/n n 1 sub def
	/y1 ED /x1 ED x1 y1 ArrowA x1 y1 moveto
	\psk@linecap\space 3 gt
		{\psk@linecap\space 0 lt {0 setlinecap} if }
		{\psk@linecap\space setlinecap} ifelse
	n {
		/y2 ED /x2 ED
		/y0 y1 def /x0 x1 def
		/length x2 x1 sub y2 y1 sub Pyth def
		\psk@dashNo\space 1.0 lt
			{/cntMax 1.0 \psk@dashNo\space div .49 add cvi def}
			{/cntMax length \psk@dashNo\space div .49 add cvi def} ifelse
		x2 x1 sub cntMax div /dx ED
		y2 y1 sub cntMax div /dy ED
		/cnt 0 def
		cntMax {
			gsave
			/x1 x1 dx add def
			/y1 y1 dy add def
			x1 y1
			cnt 2 mod 0 eq
				{ \pst@usecolor\psDashColorI }
				{ \pst@usecolor\psDashColorII } ifelse
			lineto stroke
			/cnt cnt 1 add def
			grestore
			x1 y1 moveto
		} repeat
		/y1 y2 def /x1 x2 def
	} repeat
	x0 y0 x2 y2 ArrowB L pop pop
}>
%
\def\pslineII{\pst@object{pslineII}}
\def\pslineII@i{%
    \pst@getarrows{%
        \begin@OpenObj
        \pst@getcoors[\pslineII@ii%
    }%
}
\def\pslineII@ii{%
	\addto@pscode{%
		\pst@cp
		\ifshowpoints true \else false \fi
		\tx@LineII
	}%
	\end@OpenObj%
}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pstricks-add.tex
\endinput

%% CHANGE-LOG
% v 0.9a	add relative dashNo
% v 0.9		add \pslineII
% v 0.8e	add bracePos
% v 0.8d	fix bug in arrows
% v 0.8c	small tweaks to \@@rput@iv
% v 0.8b	now every object can be passed to psbrace
% v 0.8a	fix bug with arrow
% v 0.8		ArrowFill added
% v 0.7a	adding option asolid as fillstyle
% v 0.7		ArrowInsidePos>1 for all macros
% v 0.6		ArrowInsidePos>1 sets nowthe arrows every n-th pt
% v 0.5a	small improvements to the code (use of Pyth)
% v 0.5		new psbezier and pcline to get the arrows in the right place!
% v 0.4		fix bug in psbezier and nccurve, to get the right arrow position

